Performance Asymmetry in Model-Based Reinforcement Learning

Recently, Model-Based Reinforcement Learning (MBRL) have achieved super-human level performance on the Atari100k benchmark on average. However, we discover that conventional aggregates mask a major problem, Performance Asymmetry: MBRL agents dramatically outperform humans in certain tasks (Agent-Optimal tasks) while drastically underperform humans in other tasks (Human-Optimal tasks). Indeed, despite achieving SOTA in the overall mean Human-Normalized Scores (HNS), the SOTA agent scored the worst among baselines on Human-Optimal tasks, with a striking 21X performance gap between the Human-Optimal and Agent-Optimal subsets. To address this, we partition Atari100k evenly into Human-Optimal and Agent-Optimal subsets, and introduce a more balanced aggregate, Sym-HNS. Furthermore, we trace the striking Performance Asymmetry in the SOTA pixel diffusion world model to the curse of dimensionality and its prowess on high visual detail tasks (e.g. Breakout). To this end, we propose a novel latent end-to-end Joint Embedding DIffusion (JEDI) world model that achieves SOTA results in Sym-HNS, Human-Optimal tasks, and Breakout -- thus reversing the worsening Performance Asymmetry trend while improving computational efficiency and remaining competitive on the full Atari100k.

==> figs/diamond_bias.tex <==
\begin{figure}[t]
  \centering

  % First subfigure
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pdfs/number_of_actions_count_of_shooter_games.pdf}
    \caption{Comparison of Agent-Optimal and Human-Optimal Tasks}
    \label{fig:action_space_comparison}
  \end{subfigure}
  \begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pdfs/DIAMOND_JEDI_versusAverage_Action_Shooter_Comparison.pdf}
    \caption{Overall performance of DIAMOND against other methods on tasks with Low/Large Action Space, and Non-Combat/Combat Games}  
    \label{fig:diamond_versus_others_actionspace_shooter}
  \end{subfigure}  
  \caption{\textbf{(a)} Action Space of Agent-Optimal Tasks are significantly lesser than Human-Optimal Tasks. \textbf{(b)} DIAMOND outperforms other agents on Low-Action Space tasks and Non-Combat Games while it underperforms other agents on Large-Action Space Tasks and Combat Games. .}
  % \caption{\textbf{Left:} Correlation between Combat and Non-Combat Games against Win and Losses of DIAMOND and JEDI against the averaged baselines performance on Atari100k. DIAMOND's performance has a clear high correlation and bias with the Combat/Non-Combat games whereas JEDI's performance has less bias. \textbf{Right:} DIAMOND vs. other agents in different environment settings. DIAMOND's performance bias towards Non-Action environments with Low Action Space.}
  \label{fig:action_space_combat_games_comparison}
\end{figure}




  % \quad
  % \begin{subfigure}[t]{0.33\textwidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{pdfs/action_space_action_games_corr_shooter.pdf}
  %   \caption{Overall performance of DIAMOND against other methods on tasks with Low/Large Action Space, and Non-Combat/Combat Games}  
  %   \label{fig:diamond_versus_others_actionspace_shooter}
  % \end{subfigure}  
  %   \begin{subfigure}[t]{0.33\textwidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{pdfs/action_space_action_games_corr_shooter_jedi.pdf}
  %   \caption{Overall performance of DIAMOND against other methods on tasks with Low/Large Action Space, and Non-Combat/Combat Games}  
  %   \label{fig:jedi_versus_others_actionspace_shooter}
  % \end{subfigure}  



  % \begin{subfigure}[t]{0.25\textwidth}
  %   \centering
  %   \includegraphics[width=\textwidth]{pdfs/heatmap_stacked.pdf}
  %   \caption{Number of Wins and Losses of DIAMOND and JEDI versus the averaged agent performance defined in \cref{sec:performance_bias} on Combat and Non-Combat Games. DIAMOND's performance is highly correlated to Combat/Non-Combat games while JEDI's performance is not as biased}
  %   \label{fig:diamond_jedi_number_wins_combatgames}
  % \end{subfigure}

% \begin{figure}[t]
%   \centering

%   % First subfigure
%   \begin{subfigure}[t]{0.52\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{pdfs/big_diamond_traj.pdf}

%   \end{subfigure}
%   \hfill
%   % Second subfigure
%   \begin{subfigure}[t]{0.42\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{pdfs/action_space_action_games_corr.pdf}

%   \end{subfigure}

%   \caption{\textit{Left:} Example trajectory of DIAMOND on \textit{BankHeist} displays self-sabotaging behaviour as it is unable to reason about its high complexity action space. \textit{Right:} DIAMOND vs. other agents in different environment settings. DIAMOND's performance bias towards Non-Action environments with Low Action Space.}
%   \label{fig:diamond_bad}
% \end{figure}

==> figs/hns_aggregate.tex <==

\begin{wrapfigure}{r}{0.50\textwidth}
  \vspace{-20pt} % Adjust this to align with your text
  \centering
  \includegraphics[width=\linewidth]{pdfs/jedi32_vs_baselines_HN.pdf}
  \caption{\small Mean, Median, and Interquantile Mean (IQM) is with reference to Human Normalized Scores (↑); Optimality Gap (↓) is the overall gap to human-level performance}
  \label{fig:jedi32_vs_baselines_HN}
  \vspace{-40pt} % Reduces space after figure
\end{wrapfigure}


==> figs/jedi_diamond_speed.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \vspace{-00pt}                            % tighten bottom gap (optional)
    \includegraphics[width=0.4\textwidth]{pdfs/runtime_jedi_v_diamond.pdf}
    \caption{Training curves of JEDI against DIAMOND. First row plots the performance against the environment steps. Second row plots the performance against the actual runtime duration.}
    \label{fig:jedi_vs_diamond_runtime}
   \vspace{-50pt}                            % tighten bottom gap (optional)
\end{wrapfigure}

==> figs/motivation_small.tex <==
\begin{wrapfigure}[20]{r}{0.3\textwidth}
    \centering
    \includegraphics[width=0.3\textwidth]{pdfs/fig1_starwars_cartoon.pdf}
    \caption{Asymmetry of performance on RL tasks. There exists a natural distinction between the tasks that humans are good at versus RL agents and amongst many reasons, this can be due to the reward hacking tendencies of RL or failure to learn the correct visual representations. \citep{skalse2022RewardHack, guo2021machine}}
    \label{fig:fig1_starwars_cartoon}
\end{wrapfigure}
